Partial Orders for Efficient BMC of Concurrent Software

The vast number of interleavings that a concurrent program can have is typically identified as the root cause of the difficulty of automatic analysis of concurrent software. Weak memory is generally believed to make this problem even harder. We address both issues by modelling programs' executions with partial orders rather than the interleaving semantics (SC). We implemented a software analysis tool based on these ideas. It scales to programs of sufficient size to achieve first-time formal verification of non-trivial concurrent systems code over a wide range of models, including SC, Intel x86 and IBM Power.

==> include/exp-teaser.tex <==
\section{Implementation and experiments\label{sec:implem}\label{sec:experiments}}
%2 pages

Oh what an adventure! In the next episode of \emph{Weakness as a virtue}, we'll
see how we use partial orders to verify Apache.

